Reply to: Low-frequency quantum oscillations in LaRhIn$_5$: Dirac point or nodal line?

We thank G.P. Mikitik and Yu.V. Sharlai for contributing this note and the cordial exchange about it. First and foremost, we note that the aim of our paper is to report a methodology to diagnose topological (semi)metals using magnetic quantum oscillations. Thus far, such diagnosis has been based on the phase offset of quantum oscillations, which is extracted from a "Landau fan plot". A thorough analysis of the Onsager-Lifshitz-Roth quantization rules has shown that the famous $\pi$-phase shift can equally well arise from orbital- or spin magnetic moments in topologically trivial systems with strong spin-orbit coupling or small effective masses. Therefore, the "Landau fan plot" does not by itself constitute a proof of a topologically nontrivial Fermi surface. In the paper at hand, we report an improved analysis method that exploits the strong energy-dependence of the effective mass in linearly dispersing bands. This leads to a characteristic temperature dependence of the oscillation frequency which is a strong indicator of nontrivial topology, even for multi-band metals with complex Fermi surfaces. Three materials, Cd$_3$As$_2$, Bi$_2$O$_2$Se and LaRhIn$_5$ served as test cases for this method. Linear band dispersions were detected for Cd$_3$As$_2$, as well as the $F$ $\approx$ 7 T pocket in LaRhIn$_5$.

==> preamble.tex <==
%\pdfoutput=1
\setlength{\intextsep}{10pt}
\setlength{\textfloatsep}{5pt}

%adjust height of rows in a table
\setlength\extrarowheight{2.5pt}

\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}

%% ultimate commands
	
	% align environment
			\newcommand{\e}[1]{\begin{align}{#1}\end{align}}	
	
		
	% fraction
		\newcommand{\f}[2]{\frac{#1}{#2}}
		\newcommand{\tf}[2]{\tfrac{#1}{#2}}
		
	% partial differentiation
		\newcommand{\p}[2]{\frac{\partial #1}{\partial #2}}
		\newcommand{\pf}[3]{\frac{\partial #1}{\partial #2}\bigg|_{#3}}
		\newcommand{\pa}[1]{\partial_{#1}}
		
	% label equations/sections
		\newcommand{\la}[1]{\label{#1}}

	% refer to equation, section, figure, appendix
		\newcommand{\q}[1]{Eq.\ (\ref{#1})}
		\newcommand{\qq}[2]{Eqs.\ (\ref{#1})-(\ref{#2})}
		\newcommand{\s}[1]{Sec.\ \ref{#1}}
		\newcommand{\fig}[1]{Fig.\ \ref{#1}}		
		\newcommand{\app}[1]{App.\ \ref{#1}}				
		\newcommand{\tab}[1]{Tab.\ \ref{#1}}
		\newcommand{\ocite}[1]{Ref.\ \onlinecite{#1}}
		\newcommand{\cf}[1]{[cf.\ Eq.\ (\ref{#1})]}
	
				
	% brackets
		\newcommand{\brac}[1]{\left(\;#1\;\right)}
		\newcommand{\sq}[1]{\left[\;#1\;\right]}
		\newcommand{\cu}[1]{\left\{\;#1\;\right\}}

	% insert words in equation environment

		\newcommand{\iwith}{\ins{with}}
		\newcommand{\where}{\ins{where}}		
		\newcommand{\iand}{\ins{and}}
		\newcommand{\ior}{\ins{or}}
		\newcommand{\ifor}{\ins{for}}
		\newcommand{\st}{\ins{s.t.}}
		
	% sign functions
		\newcommand{\sgn}{\text{sgn}}

	% equal, approximate, proportional signs, limits
		\newcommand{\eq}{=&\;}
		\newcommand{\condeq}[1]{\as \substack{\sma{#1}\\=}\as}
		\newcommand{\condprop}[1]{\as \substack{\sma{#1}\\ \propto}\as}
		\newcommand{\limit}[1]{\substack{\text{lim}\\#1}\as}		
		\newcommand{\appr}{\approx &\;}
		\newcommand{\prop}{\propto&\;}
		\newcommand{\define}{\as\substack{\text{def}\\ \iff}\as}					
	
	% mathbb symbols
		\newcommand{\F}{\mathbb{F}}
		\newcommand{\R}{\mathbb{R}}
		\newcommand{\Z}{\mathbb{Z}}
		\newcommand{\I}{\mathbb{I}}
		\newcommand{\C}{\mathbb{C}}
		\newcommand{\N}{\mathbb{N}}		
		\newcommand{\Q}{\mathbb{Q}}				
		\newcommand{\bbs}{\mathbb{S}}
		\newcommand{\bbt}{\mathbb{T}}

		
% for review
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

% exponential 
\newcommand{\ex}{\text{exp}}
\newcommand{\pexp}{\overline{\text{exp}}}
		
		
% plane wave
	\newcommand{\eikr}{e^{i\bk \cdot \br}}
	\newcommand{\eikR}{e^{i\bk \cdot \bR}}
	\newcommand{\emikr}{e^{-i\bk \cdot \br}}
	\newcommand{\emikR}{e^{-i\bk \cdot \bR}}	

% divergence,curl,laplacian
\newcommand{\na}{\nabla}
\newcommand{\nai}{\nabla_i}
\newcommand{\naj}{\nabla_j}
\newcommand{\nak}{\nabla_k}
\newcommand{\nal}{\nabla_l}
\newcommand{\diverge}{\nabla \cdot}
\newcommand{\curl}{\nabla \times}
\newcommand{\lap}{\nabla^2}
\newcommand{\nabr}{\nabla_{\boldsymbol{r}}}
\newcommand{\nabk}{\nabla_{\boldsymbol{k}}}
\newcommand{\nabkp}{\nabla_{\boldsymbol{k}'}}

%fundamental constants
\newcommand{\bohr}{\mu_{\sma{B}}}
\newcommand{\gfac}{g_{\sma{0}}}
\newcommand{\lmt}{l^{\mt}}
\newcommand{\lmf}{l^{\text{-}4}}
\newcommand{\lmo}{l^{\mo}}




% specific to geometric_orbital
\newcommand{\om}{orbital moment }
\newcommand{\omm}{orbital moment}
\newcommand{\zf}{Zilberman-Fischbeck }
\newcommand{\checkgp}{\check{g}^{\sma{\perp}}}
\newcommand{\btperp}{$BT_{\sma{\perp}}$}
\newcommand{\bise}{Bi$_2$Se$_3$}



% c creation operators

\newcommand{\cdagk}{\dg{c}_{\bk}}
\newcommand{\ck}{\pdg{c}_{\bk}}
\newcommand{\cdagksig}{\dg{c}_{\bk,\sigma}}
\newcommand{\cksig}{\pdg{c}_{\bk,\sigma}}
\newcommand{\cdagkup}{c^\dagger_{\boldsymbol{k}\uparrow}}
\newcommand{\cdagkdo}{c^\dagger_{\boldsymbol{k}\downarrow}}
\newcommand{\ckup}{\pdg{c}_{\boldsymbol{k} \uparrow}}
\newcommand{\ckdo}{\pdg{c}_{\boldsymbol{k} \downarrow}}

\newcommand{\cdag}[1]{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{#1}}}
\newcommand{\cnod}[1]{c_{\scriptstyle{#1}}}


\newcommand{\cdj}{c^{\scriptscriptstyle{\dagger}}_{\scriptstyle{j \sigma}}}
\newcommand{\cnj}{c_{\scriptstyle{j' \sigma'}}}


% f creation operator

\newcommand{\fsig}{\pdg{f}_{\sigma}}
\newcommand{\fdagsig}{\dg{f}_{\sigma}}
\newcommand{\fup}{\pdg{f}_{\uparrow}}
\newcommand{\fdagup}{\dg{f}_{\uparrow}}
\newcommand{\fdo}{\pdg{f}_{\downarrow}}
\newcommand{\fdagdo}{\dg{f}_{\downarrow}}


%levi Cevita
\newcommand{\levi}[1]{\epsilon_{#1}}


%spin symbols
\newcommand\nup{\hat{n}_{f\uparrow}}
\newcommand\ndo{\hat{n}_{f\downarrow}}
\newcommand\avenup{{n}_{f\uparrow}}
\newcommand\avendo{{n}_{f\downarrow} }

% energies with varepsilon
\newcommand{\var}{\varepsilon}
%\newcommand{\var}[1]{\varepsilon_{#1}}
\newcommand{\efu}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\uparrow}}}
\newcommand{\efd}{\varepsilon_{\scriptscriptstyle{F}}^{\scriptscriptstyle{\downarrow}}}
\newcommand{\ef}{\varepsilon_{\scriptscriptstyle{f}}}
\newcommand{\EF}{E_{\scriptscriptstyle{F}}}
\newcommand{\ek}{\varepsilon_{\boldsymbol{k}}}
\newcommand{\eF}{\varepsilon_{\scriptscriptstyle{F}}}
\newcommand{\enk}{\varepsilon_{n,\bk}}




% space

\newcommand\as{\;\;\;\;}
\newcommand\ass{\;\;\;\;\;\;\;\;}


\newcommand\Wline[2]{ \pdg{\W}_{\sma{#1 \leftarrow #2}}}


%hat operators

\newcommand{\hn}{\hat{n}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hPi}{\hat{{\Pi}}}
\newcommand{\hpsi}{\hat{{\psi}}}
\newcommand{\hphi}{\hat{{\phi}}}
\newcommand{\hrho}{\hat{{\rho}}}
\newcommand{\hsigma}{\hat{{\sigma}}}
	%hatted operators with dagger
	\newcommand{\dhpsi}{\dg{\hat{{\psi}}}}
	\newcommand{\dhphi}{\dg{\hat{{\phi}}}}


%hatted bold symbols
\newcommand{\hbp}{\hat{\bp}}
\newcommand{\hbr}{\hat{\br}}
\newcommand{\hbv}{\hat{\bv}}
\newcommand{\hbx}{\hat{\bx}}
\newcommand{\bhp}{\boldsymbol{\hat{p}}}
\newcommand{\hbA}{\hat{\bA}}
\newcommand{\hbB}{\hat{\bB}}
\newcommand{\hbJ}{\hat{\bJ}}
\newcommand{\hbP}{\hat{\bP}}
\newcommand{\hbpi}{\hat{\boldsymbol{\pi}}}
\newcommand{\hbPi}{\hat{\boldsymbol{\Pi}}}


%bold symbols

\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bkp}{\boldsymbol{k}_{\sma{\perp}}}
\newcommand{\bkpar}{\bk_{\parallel}}
\newcommand{\bkone}{\boldsymbol{k_1}}
\newcommand{\bktwo}{\boldsymbol{k_2}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\brp}{\boldsymbol{r}_{\sma{\perp}}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bze}{\boldsymbol{0}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bcalf}{\boldsymbol{\calf}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarpi}{\boldsymbol{\varpi}}
\newcommand{\bdeltapar}{\boldsymbol{\delta}_{\sma{\parallel}}}
\newcommand{\bna}{\boldsymbol{\nabla}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}



%\mathfrak
\newcommand{\frake}{\mathfrak{e}}
\newcommand{\frako}{\mathfrak{o}}
\newcommand{\frakt}{\mathfrak{t}}
\newcommand{\fraks}{\mathfrak{s}}
\newcommand{\frakr}{\mathfrak{r}}
\newcommand{\mx}{\mathfrak{X}}
\newcommand{\mxx}{\mathfrak{X}^x}
\newcommand{\mxy}{\mathfrak{X}^y}
\newcommand{\bmx}{\bar{M}_x}


\newcommand{\orb}{\boldsymbol{\mathfrak{A}}}
\newcommand{\lutt}{\boldsymbol{\mathfrak{L}}}



%tilde
\newcommand{\tbPi}{\tilde{\bPi}}
\newcommand{\tPi}{\tilde{\Pi}}
\newcommand{\txi}{\tilde{\xi}}
\newcommand{\tbv}{\tilde{\bv}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tbmx}{\tilde{\bmx}}
\newcommand{\tmxx}{\tilde{\mx}^x}
\newcommand{\tmxy}{\tilde{\mx}^y}
\newcommand{\tmx}{\tilde{\mx}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tbsigma}{\tilde{\bsigma}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\tilu}[1]{\tilde{u}_{#1}}
\newcommand\tilX{\tilde{X}}
\newcommand\tilZ{\tilde{Z}}
\newcommand\tilGamma{\tilde{\Gamma}}
\newcommand\tilU{\tilde{U}}

%calligraphic
\newcommand{\calL}{{\cal L}}
\newcommand{\W}{{\cal W}}
\newcommand{\A}{{\cal A}}


% equal signs
\newcommand\kzeq{\;\stackrel{\mathclap{\normalfont\mbox{$\sma{\bar{k}_z}$}}}{=}\;}

%breve 
\newcommand{\breveg}{\breve{g}}


% symmetry operators
\newcommand{\inv}{\mathfrak{i}}
\newcommand{\mir}{\mathfrak{r}}
\newcommand\glide{\mathfrak{g}}
\newcommand\rot{\mathfrak{c}}
\newcommand\scr{\mathfrak{s}}
\newcommand\tra{\mathfrak{t}}


\newcommand{\calti}{{\cal T}_{\sma{\cal I}}}
\newcommand{\gdel}{g_{\boldsymbol{\delta}}}
\newcommand{\pgdel}{\pdg{g}_{\boldsymbol{\delta}}}
\newcommand{\bmz}{\bar{M}_z}
\newcommand{\calbmx}{{\cal \bar{M}}_x}
\newcommand{\calgdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevegdel}{\pdg{\breve{g}}_{\sma{\bdelta}}}
\newcommand{\brevebmx}{\breve{\bar{M}}_x}
\newcommand{\uit}{U_{\sma{\cali T}}}
\newcommand{\utg}{U_{\sma{Tg \bdelta}}}
\newcommand{\ut}{U_{\sma{T}}}
\newcommand{\ug}{U_{\sma{g \bdelta}}}
\newcommand{\ubmx}{U_{\sma{\bmx}}}
\newcommand{\utbmz}{U_{\sma{T\bmz}}}
\newcommand{\calug}{\calg_{\sma{\bdelta}}}
\newcommand{\caluit}{\calu_{\sma{\cali T}}}
\newcommand{\caltgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetgdel}{\breve{T}_{\sma{g \bdelta}}}
\newcommand{\brevetbmx}{\breve{T}_{\sma{\bmx}}}
\newcommand{\hattbmx}{\hat{T}_{\sma{\bmx}}}
\newcommand{\brevetbmz}{\breve{T}_{\sma{\bmz}}}
\newcommand{\breveti}{\breve{T}_{\sma{\cali}}}
\newcommand{\caltbmz}{\calt_{\sma{\bmz}}}
\newcommand{\caltbmx}{\calt_{\sma{\bmx}}}
\newcommand{\calut}{\calu_{\sma{T}}}
\newcommand{\hatgdel}{\pdg{\hat{g}}_{\sma{\bdelta}}}
\newcommand{\hatTg}{\pdg{\hat{T}}_{\sma{g\bdelta}}}
\newcommand\csixdel{C_{\sma{6,\bdelta}}}
\newcommand\brevecsixdel{\breve{C}_{\sma{6,\bdelta}}}
\newcommand\cthreedel{C_{\sma{3,\bdelta}}}
\newcommand\brevecthreedel{\breve{C}_{\sma{3,\bdelta}}}
\newcommand\hatcthreedel{\hat{C}_{\sma{3,\bdelta}}}
\newcommand\cthreetwodel{C_{\sma{3,2\bdelta}}}
\newcommand\brevecthreetwodel{\breve{C}_{\sma{3,2\bdelta}}}
\newcommand\brevectwothreedel{\breve{C}_{\sma{2,3\bdelta}}}
\newcommand\ctwothreedel{C_{\sma{2,3\bdelta}}}
\newcommand\hatcsixdel{\hat{C}_{\sma{6,\bdelta}}}
\newcommand\ucsixdel{U_{\sma{C_6,\bdelta}}}
\newcommand\cndel{C_{\sma{n,\bdelta}}}
\newcommand\cbarndel{C_{\sma{\bar{n},\bdelta}}}
\newcommand\ucndel{U_{\sma{C_n,\bdelta}}}
\newcommand\hatcndel{\hat{C}_{\sma{n,\bdelta}}}
\newcommand\brevecndel{\breve{C}_{\sma{n,\bdelta}}}
\newcommand\brevectwotwodel{\breve{C}_{\sma{2,2\bdelta}}}
\newcommand\brevecfourdel{\breve{C}_{\sma{4,\bdelta}}}
\newcommand\brevectwodel{\breve{C}_{\sma{2,\bdelta}}}


% vectors and matrices
\newcommand{\vectwo}[2]{\begin{pmatrix} {#1}\\{#2} \end{pmatrix}}
\newcommand{\matrixtwo}[4]{\begin{pmatrix} #1 & #2 \\ #3 & #4 \end{pmatrix}}
\newcommand{\diagmatrix}[2]{\begin{pmatrix} #1 & 0 \\ 0 & #2 \end{pmatrix}}
\newcommand{\matrixthree}[9]{\begin{pmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{pmatrix}}


% Pauli matrices
\newcommand{\szero}{\sigma_{\sma{0}}}
\newcommand{\sx}{\sigma_{\sma{1}}}
\newcommand{\sy}{\sigma_{\sma{2}}}
\newcommand{\sz}{\sigma_{\sma{3}}}
\newcommand{\tzero}{\tau_{\sma{0}}}
\newcommand{\tx}{\tau_{\sma{1}}}
\newcommand{\ty}{\tau_{\sma{2}}}
\newcommand{\tz}{\tau_{\sma{3}}}



% parafermion operators
\newcommand{\gt}{\gamma_{\sma{2}}}
\newcommand{\gth}{\gamma_{\sma{3}}}
\newcommand{\gfo}{\gamma_{\sma{4}}}
\newcommand{\gfi}{\gamma_{\sma{5}}}
\newcommand{\gj}{\gamma_{\sma{j}}}
\newcommand{\gtj}{\gamma_{\sma{2j}}}
\newcommand{\gtjpo}{\gamma_{\sma{2j+1}}}
\newcommand{\gtjpt}{\gamma_{\sma{2j+2}}}
\newcommand{\gtjmo}{\gamma_{\sma{2j-1}}}
\newcommand{\gtL}{\gamma_{\sma{2L}}}
\newcommand{\gtLpo}{\gamma_{\sma{2L+1}}}
\newcommand{\gtLpt}{\gamma_{\sma{2L+2}}}
\newcommand{\gtLmo}{\gamma_{\sma{2L-1}}}
\newcommand{\gtLmt}{\gamma_{\sma{2L-2}}}
\newcommand{\gtLmth}{\gamma_{\sma{2L-3}}}
\newcommand{\gtLmfo}{\gamma_{\sma{2L-4}}}


% insert text in equation
\newcommand{\ins}[1]{\;\;\;\;\text{#1}\;\;\;\;}


%momentum parallel and perpendicular
\newcommand{\kpar}{\boldsymbol{k}_{{\shortparallel}}}
\newcommand{\Dpar}{D^{g}_{{\shortparallel}}}
\newcommand{\kper}{k_{\perp}}


% Cnv 
\newcommand{\ctv}{C_{3v}}
\newcommand{\cfv}{C_{4v}}
\newcommand{\csv}{C_{6v}}
\newcommand{\cnv}{C_{nv}}


%C_n Time-reversal
\newcommand{\cnt}{C_n {\cal T}}
\newcommand{\cn}{C_n}
\newcommand{\cfour}{C_4}
\newcommand{\cs}{C_6}
\newcommand{\ct}{C_3}
\newcommand{\cst}{C_6{\cal T}}
\newcommand{\cft}{C_4{\cal T}}
\newcommand{\ctt}{C_2{\cal T}}


% average 
\newcommand{\ave}[1]{\langle\,#1\,\rangle}



%inverse Angstroms and Angstroms
\newcommand{\invA}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}
\newcommand{\ang}{\mathrm{\AA}}

% Lagrangian
\newcommand{\lag}{{\mathscr{L}}}


% green's function
\newcommand{\green}{{\mathscr{G}}}

% Cauchy principal value
\newcommand{\prin}{{\mathscr{P}}}

% imaginary and real parts
\newcommand{\imag}{{\mathscr{I}}}
\newcommand{\real}{{\mathscr{R}}}


%total differentiation
\newcommand{\totaldif}[2]{\frac{ d #1}{d #2}}

% calligraphic font
\newcommand{\cala}{{\cal A}}
\newcommand{\calb}{{\cal B}}
\newcommand{\calc}{{\cal C}}
\newcommand{\cald}{{\cal D}}
\newcommand{\cale}{{\cal E}}
\newcommand{\calf}{{\cal F}}
\newcommand{\calg}{{\cal G}}
\newcommand{\calh}{{\cal H}}
\newcommand{\tcalh}{\tilde{\cal H}}
\newcommand{\cali}{{\cal I}}
\newcommand{\calj}{{\cal J}}
\newcommand{\calk}{{\cal K}}
\newcommand{\call}{{\cal L}}
\newcommand{\calm}{{\cal M}}
\newcommand{\caln}{{\cal N}}
\newcommand{\calo}{{\cal O}}
\newcommand{\calp}{{\cal P}}
\newcommand{\calq}{{\cal Q}}
\newcommand{\calr}{{\cal R}}
\newcommand{\cals}{{\cal S}}
\newcommand{\calt}{{\cal T}}
\newcommand{\calu}{{\cal U}}
\newcommand{\calv}{{\cal V}}
\newcommand{\calw}{{\cal W}}
\newcommand{\calx}{{\cal X}}
\newcommand{\caly}{{\cal Y}}
\newcommand{\calz}{{\cal Z}}

% mathscript font
\newcommand{\scra}{{\mathscr A}}
\newcommand{\scrb}{{\mathscr B}}
\newcommand{\scrc}{{\mathscr C}}
\newcommand{\scrd}{{\mathscr D}}
\newcommand{\scre}{{\mathscr E}}
\newcommand{\barscre}{\bar{\mathscr E}}
\newcommand{\scrf}{{\mathscr F}}
\newcommand{\scrg}{{\mathscr G}}
\newcommand{\scrh}{{\mathscr H}}
\newcommand{\tscrh}{\tilde{\mathscr H}}
\newcommand{\scri}{{\mathscr I}}
\newcommand{\scrj}{{\mathscr J}}
\newcommand{\scrk}{{\mathscr K}}
\newcommand{\scrl}{{\mathscr L}}
\newcommand{\scrm}{{\mathscr M}}
\newcommand{\scrn}{{\mathscr N}}
\newcommand{\scro}{{\mathscr O}}
\newcommand{\scrp}{{\mathscr P}}
\newcommand{\scrq}{{\mathscr Q}}
\newcommand{\scrr}{{\mathscr R}}
\newcommand{\scrs}{{\mathscr S}}
\newcommand{\scrt}{{\mathscr T}}
\newcommand{\scru}{{\mathscr U}}
\newcommand{\scrv}{{\mathscr V}}
\newcommand{\scrw}{{\mathscr W}}
\newcommand{\scrx}{{\mathscr X}}
\newcommand{\scry}{{\mathscr Y}}
\newcommand{\scrz}{{\mathscr Z}}


%Gamma matrices
\newcommand{\gam}[1]{\Gamma_{#1}}

%determinant
\newcommand{\de}[1]{\text{det}[\;#1\;]}

%trace
\newcommand{\tr}{\text{Tr}}




\newcommand{\noi}[1]{\noindent (#1)}
\newcommand{\imp}{\;\;\Rightarrow\;\;}
\newcommand{\mo}{\text{-}1}
\newcommand{\mt}{\text{-}2}
\newcommand{\minus}{\text{-}}
\newcommand{\oneover}[1]{\tfrac{1}{#1}}


% A command for inner product and bras and kets
\newcommand{\braket}[2]{\big\langle #1 \big| #2 \big\rangle}
\newcommand{\ketbra}[2]{\big|  #1  \big\rangle \big\langle #2 \big| }
\newcommand{\braopket}[3]{\big\langle #1 \big| #2 \big| #3 \big\rangle}
\newcommand{\bra}[1]{\big\langle#1\big|}
\newcommand{\ket}[1]{\big|#1\big\rangle}
\newcommand{\bigket}[1]{\bigl|#1\bigr\rangle}
\newcommand{\textket}[1]{|#1\rangle}
  %double bras and kets
	\newcommand{\dbraket}[2]{\big\langle\big\langle #1 \big| #2 \big\rangle \big\rangle}
  \newcommand{\dketbra}[2]{\big|  #1  \big\rangle\big\rangle \big\langle \big\langle #2 \big| }
  \newcommand{\dbraopket}[3]{\big\langle \big\langle #1 \big| #2 \big| #3 \big\rangle \big\rangle}
  \newcommand{\dket}[1]{\big|#1\big\rangle \big\rangle}
  \newcommand{\dbra}[1]{\big\langle \big\langle#1\big|}
  \newcommand{\dexp}[1]{\big\langle\big\langle #1 \big\rangle \big\rangle}



% Various bracketing commands
\newcommand{\of}[1]{\!\left(#1\right)}
\newcommand{\sqof}[1]{\left[#1\right]}
\newcommand{\cuof}[1]{\left\{#1\right\}}

% commutator and anticommutator
\newcommand{\comm}[2]{\left[#1,#2\right]}
\newcommand{\anticomm}[2]{\left\{#1,#2\right\}}
% sum on nearest neighbor bonds
\newcommand{\bond}{\left\langle i, j \right\rangle}
%\newcommand{\bondsum}{\sum_{\left\langle i, j \right\rangle}}
\newcommand{\nbond}{\left\langle\left\langle i, j \right\rangle\right\rangle}
% 1/2
\newcommand{\half}{\frac{1}{2} }
\newcommand{\thalf}{\tfrac{1}{2} }
% simplifies using the up and down arrows to denote spin
\newcommand{\up}{\uparrow}
\newcommand{\down}{\downarrow}
% Absolute value  
\newcommand{\abs}[1]{\left|#1\right|}

% Roman functions for real and imaginary parts
\newcommand{\re}{\mathrm{Re}}
\newcommand{\im}{\mathrm{Im}}


%Expectation values
\newcommand{\expect}[1]{\left\langle#1\right\rangle}
\newcommand{\pdag}{\phantom{\dagger}}
\newcommand{\pdg}[1]{{#1}^{\phantom{\dagger}}}

\newcommand{\bkap}{\bar{\glide}}
\newcommand{\bchi}{\bar{\chi}}
\newcommand{\baeta}{\bar{\eta}}
\newcommand{\lin}{\notag \\}



\newcommand{\ab}{\alpha\beta}
\newcommand{\deli}{\Delta^{-1}}


\newcommand{\ra}{{R\,\alpha}}
\newcommand{\rax}{{R+\vec{x}\,\alpha}}

\newcommand{\rb}{{R'\,\beta}}
\newcommand{\rarb}{{R\,\alpha};R'\,\beta}
\newcommand{\zth}{\mathbb{Z}_3}


\newcommand{\xin}{x_{\tex{inv}}}
\newcommand{\low}{L$\ddot{\text{o}}$wdin\;}
\newcommand{\tex}[1]{\sma{\text{#1}}}











\newcommand{\kf}{k_{\scriptscriptstyle{F}}}

\newcommand{\bfk}{\boldsymbol{k}}
\newcommand{\bfq}{\boldsymbol{q}}



\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\nk}{n_{\boldsymbol{k}'}}
\newcommand{\dk}{\Delta_{\boldsymbol{k}'}}
\newcommand{\Dk}{\Delta_{\boldsymbol{k}}}
\newcommand{\tk}{\tilde{k}}
\newcommand{\tkp}{\tilde{k}'}
\newcommand{\bal}{\begin{align}}
\newcommand{\Ainv}{\mathrm{\AA^{\scriptscriptstyle{-1}}}}

\newcommand{\V}{V_{\text{eff}}}
\newcommand{\si}{\;\text{sin}\,}
\newcommand{\ta}{\;\text{tan}\,}
\newcommand{\co}{\;\text{\text{cos}}\,}
\newcommand{\te}{t_{\text{eff}}}
\newcommand{\ep}{\bar{\epsilon}}



\newcommand{\braa}[1]{\left\langle#1\right|_{\scriptscriptstyle{A}}}
\newcommand{\brab}[1]{\left\langle#1\right|_{\scriptscriptstyle{B}}}

\newcommand{\dg}[1]{#1^{\scriptstyle{\dagger}}}
\newcommand{\bof}[1]{\boldsymbol{#1}}
\newcommand{\sma}[1]{\scriptscriptstyle{#1}}
\newcommand{\po}{{\sma{+}} 1}



\newcommand{\noc}{n_{\sma{{occ}}}}
\newcommand{\ntot}{n_{\sma{{tot}}}}

\newtheorem{definition}{Definition}[section]
